Video Action Understanding

Many believe that the successes of deep learning on image understanding problems can be replicated in the realm of video understanding. However, due to the scale and temporal nature of video, the span of video understanding problems and the set of proposed deep learning solutions is arguably wider and more diverse than those of their 2D image siblings. Finding, identifying, and predicting actions are a few of the most salient tasks in this emerging and rapidly evolving field. With a pedagogical emphasis, this tutorial introduces and systematizes fundamental topics, basic concepts, and notable examples in supervised video action understanding. Specifically, we clarify a taxonomy of action problems, catalog and highlight video datasets, describe common video data preparation methods, present the building blocks of state-of-the art deep learning model architectures, and formalize domain-specific metrics to baseline proposed solutions. This tutorial is intended to be accessible to a general computer science audience and assumes a conceptual understanding of supervised learning.

==> updated-table3.tex <==
\begin{table*}
    \footnotesize
    \centering
    \caption{Prominent Video Action Understanding Challenges 2013-2021.}
    \setlength{\tabcolsep}{5pt}
    \begin{tabular}{| l c l l l l l l |}
        \hline
         Workshop & Year & Conf. & Problem & Dataset & Metric(s) & Top Result & \#Teams \\
         \hline
         % https://www.crcv.ucf.edu/ICCV13-Action-Workshop/
         THUMOS \cite{THUMOS13} & 2013 & ICCV & AR & UCF101 & average accuracy & 85.90 \cite{Wang2013LEARINRIASF} & 17 \\
          & & & SAL/D & UCF101-24 & ROC AUC sIoU@0.2 & n/a & n/a \\
          \hline
         % https://www.crcv.ucf.edu/THUMOS14/submission.html
         THUMOS \cite{THUMOS14} & 2014 & ECCV & AR & UCF101+ & mAP & 0.71 \cite{Jain2014UniversityOA} & 11 \\
          & & & TAL/D & UCF101-20 & mAP tIoU@\{0.1,0.2,0.3,0.4,0.5\} & .4,.3,.3,.2,.1 \cite{Oneata2014TheLS} & 3 \\
          \hline
         % http://www.thumos.info/
         % https://arxiv.org/abs/1604.06182v1
         THUMOS \cite{THUMOS15, idrees2017thumos} & 2015 & CVPR & AR & UCF101+1 & mAP & 0.74 \cite{uts2016} & 11 \\
          & & & TAL/D & UCF101-20 & mAP tIoU@\{0.1,0.2,0.3,0.4,0.5\} & .4,.4,.3,.2,.2 \cite{Yuan2015ADSCSA} & 1 \\
          \hline
         % http://activity-net.org/challenges/2016/index.html
         % http://activity-net.org/challenges/2016/data/anet_challenge_summary.pdf
         ActivityNet \cite{Heilbron_2015_CVPR} & 2016 & CVPR & AR & ActivityNet 1.3 & mAP, Top-1 accuracy, Top-3 accuracy & 93.2, 88.1 \cite{xiong2016cuhk} & 26 \\
          & & & TAL/D & ActivityNet 1.3 & mAP-50, mAP-75, average-mAP & 42.5 & 6 \\
          \hline
         % http://activity-net.org/challenges/2017/index.html
         % https://arxiv.org/abs/1710.08011
         ActivityNet \cite{ghanem2017activitynet} & 2017 & CVPR & AR & ActivityNet 1.3 & Top-1 error & 8.8 \cite{ghanem2017activitynet} & n/a \\
          & & & AR & Kinetics-400 & average(Top-1 error, Top-5 error) & 12.4 \cite{bian2017revisiting} & 31 \\
          & & & TAP & ActivityNet 1.3 & AR-AN AUC & 64.80 \cite{lin2018temporal} & 17 \\
          & & & TAL/D & ActivityNet 1.3 & mAP tIoU@0.5:0.05:0.95 & 33.40 \cite{lin2018temporal} & 17 \\
          \hline
         % http://activity-net.org/challenges/2018/challenge.html
         % https://arxiv.org/abs/1808.03766
         ActivityNet \cite{ghanem2018activitynet} & 2018 & CVPR & AR & Kinetics-600 & average(Top-1 error, Top-5 error) & 10.99 \cite{he2018exploiting} & 13 \\
          & & & AR & MiT (full-track) & average(Top-1 acc, Top-5 acc) & 52.91 \cite{li2018team} & 29 \\
          & & & AR & MiT (mini-track) & average(Top-1 acc, Top-5 acc) & 47.72 \cite{guansysu} & 12 \\
          & & & TAP & ActivityNet 1.3 & AR-AN AUC & 71.0 \cite{ghanem2018activitynet} & 55 \\
          & & & TAL/D & ActivityNet 1.3 & mAP tIoU@0.5:0.05:0.95 & 38.53 \cite{Lin_2018_ECCV} & 43 \\
          & & & SAL/D & AVA & frame-mAP sIoU@0.5 & 20.99 \cite{ava2018topresult} & 23 \\
          \hline
         % http://activity-net.org/challenges/2019/challenge.html
         ActivityNet \cite{activitynetchallenge2019, Lee_2020_WACV} & 2019 & CVPR & AR & Kinetics-700 & average(Top-1 error, Top-5 error) & 17.88 \cite{qiu2019trimmed} & 15 \\
          & & & AR & EPIC-KITCHENS-55 & micro-avg Top-1,5 acc, macro-AP,AR & 41.4, 25.1 \cite{wang2019baiduuts} & 25 \\
          & & & AP & EPIC-KITCHENS-55 & micro-avg Top-1,5 acc, macro-AP,AR & 13.2, 8.5 \cite{Furnari_2019_ICCV} & 8 \\
          & & & TAP & ActivityNet 1.3 & AR-AN AUC & 72.99 & 61 \\
          & & & TAL/D & ActivityNet 1.3 & mAP tIoU@0.5:0.05:0.95 & 39.7 & 23 \\
          & & & TAL/D & VIRAT & P$_{rate}$@miss$_{FA}$ & 0.605 & 42 \\ % \cite{actev-results-2019}
          & & & SAL/D & AVA & frame mAP sIoU@0.5 & 34.25 \cite{Feichtenhofer_2019_ICCV} & 32 \\
          \hline
         % https://sites.google.com/view/multimodalvideo/home
         Multi-modal \cite{multimodalICCV19} & 2019 & ICCV & AR & Multi-MiT & mAP & 0.608 \cite{zhang2020top1} & 10 \\
          & & & TAL/D & HACS Segments & mAP tIoU@0.5:0.05:0.95 & 23.49 \cite{zhang2019learning} & 5 \\
          \hline
         % http://activity-net.org/challenges/2020/index.html
         ActivityNet \cite{activitynetchallenge2020} & 2020 & CVPR & AR & Kinetics-700 & average(Top-1 error, Top-5 error) & 14.9 & 4 \\
          & & & TAL/D & ActivityNet 1.3 & mAP tIoU@0.5:0.05:0.95 & 42.79 \cite{wang2020cbrnet} & 55 \\
          & & & TAL/D & MEVA \cite{Corona_2021_WACV} & avg(1-$P_{\text{miss}}$) across TFA from 0-20\% & 0.350 & 11 \\ % \cite{actev-results-2020}
          & & & TAL/D & HACS Segments & mAP tIoU@0.5:0.05:0.95 & 40.53 \cite{qing2020temporal} & 22 \\
          & & & TAL/D & HACS Clips+Seg. & mAP tIoU@0.5:0.05:0.95 & 39.29 \cite{gaomulti} & 13 \\
          & & & SAL/D & AVA-Kinetics & frame mAP sIoU@0.5 & 39.62 \cite{chen20201st} & 11 \\
          \hline
          % http://activity-net.org/challenges/2021/
          ActivityNet & 2021 & CVPR & AR & Kinetics-700-2020 \cite{DBLP:journals/corr/abs-2010-10864} & average(Top-1 error, Top-5 erro) & 14.0 & 27 \\
          & & & AR & TinyVIRAT \cite{demir2020tinyvirat} & F1-score & 0.478 \cite{tirupattur2021tinyaction} & 3+ \\
          & & & TAL/D & ActivityNet 1.3 & mAP tIoU@0.5:0.05:0.95 & 44.67 \cite{DBLP:journals/corr/abs-2106-11812} & 3+ \\
          & & & TAL/D & HACS Segments & mAP tIoU@0.5:0.05:0.95 & 44.29 \cite{DBLP:journals/corr/abs-2106-13014} & 22 \\
          & & & TAL/D & HACS Clips+Seg. & mAP tIoU@0.5:0.05:0.95 & 22.45 \cite{DBLP:journals/corr/abs-2106-13014} & 13 \\
          & & & TAL/D & SoccerNet-V2 \cite{deliege2021soccernetv2} & average mAP per class & 74.84 \cite{zhoukangcheng2021} & 7 \\
          & & & TAL/D & MEVA & avg(1-$P_{\text{miss}}$) across TFA from 0-20\% & 0.425 & 9 \\
          & & & SAL/D & AVA-Kinetics & frame mAP sIoU@0.5 & 40.67 \cite{DBLP:journals/corr/abs-2106-08061} & 11 \\
         \hline
         %\multicolumn{7}{l}{AR = Action Recognition} \\
         %\multicolumn{7}{l}{TAP = Temporal Action Proposal} \\
         %\multicolumn{7}{l}{TAL/D = Temporal Action Localization/Detection} \\
         %\multicolumn{7}{l}{SAL/D = Spatiotemporal Action Localization/Detection} \\
    \end{tabular}
    \label{tab:app-competitions}
\end{table*}
